MambaMOT: State-Space Model as Motion Predictor for Multi-Object Tracking

In the field of multi-object tracking (MOT), traditional methods often rely on the Kalman filter for motion prediction, leveraging its strengths in linear motion scenarios. However, the inherent limitations of these methods become evident when confronted with complex, nonlinear motions and occlusions prevalent in dynamic environments like sports and dance. This paper explores the possibilities of replacing the Kalman filter with a learning-based motion model that effectively enhances tracking accuracy and adaptability beyond the constraints of Kalman filter-based tracker. In this paper, our proposed method MambaMOT and MambaMOT+, demonstrate advanced performance on challenging MOT datasets such as DanceTrack and SportsMOT, showcasing their ability to handle intricate, non-linear motion patterns and frequent occlusions more effectively than traditional methods.

==> table/dancetrack-val.tex <==
\begin{table*}[t]
\caption{Performance comparison of different motion models on DanceTrack validation set. We implemented most of the motion models (besides MLP) with similar model size for fair comparison in the motion modeling task. KF stands for Kalman filter. 
}
\vspace{-6pt}
  \begin{center}
    {\small{
\begin{tabular}{l | c | cccccc}
% \toprule
% \multicolumn{6}{c}{DanceTrack - Val} \\
\toprule
Module & ~$\#$ Param~ &~HOTA & DetA & AssA & IDF1 & MOTA\\
\midrule
IoU & - & 44.7 & 79.6 & 25.3 & 36.8 & 87.3\\
KF & - & 47.8 & 74.0 & 31.0 & 48.3 & 88.2\\
MLP & 6K & 48.7 & 77.0 & 31.0 & 46.7 & 87.3\\ 
RNN & 0.2M & 50.0 & 77.4 & 32.5 & 47.8 & 87.4\\
LSTM & 0.2M & 50.4 & 77.2 & 33.0 & 48.7 & 87.3\\
Transformer~ & 0.2M & 51.8 & \textbf{77.6} & 34.8 & \textbf{50.5} & \textbf{87.6}\\
Mamba & 0.2M & \textbf{52.1} & \textbf{77.6} & \textbf{35.1} & 49.2 & 87.4\\

\bottomrule
\end{tabular}
}}
\end{center}
\label{table:dance-val}
\end{table*}


==> table/ids.tex <==
\begin{table}[h]
\caption{Overall Comparison with several Kalman filter-based trackers on SportsMOT. Blue row is our proposed MambaMOT\textsuperscript{+}. All the methods are evaluated based on the same detections.}
\vspace{-6pt}
  \begin{center}
    {\small{
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
Methods & HOTA~($\uparrow$) & DetA~($\uparrow$) & AssA~($\uparrow$) & IDF1~($\uparrow$) & MOTA~($\uparrow$) & IDs~($\downarrow$) \\
\midrule
ByteTrack \cite{zhang2022bytetrack} & 62.0 & 77.0 & 49.9 & 68.7 & 93.9 & 5,040 \\
OC-SORT \cite{cao2023observation} & 70.2 & 85.9 & 57.4 & 70.4 & 93.9 & 4,834 \\

\rowcolor{aliceblue}
MambaMOT\textsuperscript{+} & \textbf{71.3} & \textbf{86.7} & \textbf{58.6} & \textbf{71.1} & \textbf{94.9} & \textbf{4,445}\\

\bottomrule
\end{tabular}
}}}
\end{center}
\label{table:ids}
\end{table} 

==> table/mot17-matching.tex <==
\begin{table*}[t]
\caption{Ablation study on the effect of \textbf{Different Matching Cost} on MOT17, DanceTrack and SportsMOT, we conduct different matching cost including the $IoU$ along with $L1$ and $L2$. }
\vspace{-6pt}
  \begin{center}
    {
\begin{tabular}{c|ccc|cccccc}
% \toprule
% \multicolumn{6}{c}{DanceTrack - Val} \\
\toprule 

 \hspace{.5em} Dataset \hspace{.5em} &
 \hspace{.5em}$IoU$\hspace{.5em} & \hspace{.5em}$L1$\hspace{.5em} & \hspace{.5em}$L2$\hspace{.5em} & HOTA & IDF1 & AssA & MOTA & DetA \\
\midrule

\multirow{3}{*}{MOT17} & $\checkmark$ & & &  65.5 & 75.3 & 66.3 & 76.9 & 65.2 \\
& $\checkmark$ & $\checkmark$ & & \textbf{66.9} &\textbf{77.2} & \textbf{66.4} & 76.9 &  \textbf{67.9} \\
& $\checkmark$ & & $\checkmark$ & 65.4 & 73.3 & 66.3 & 76.8 & 65.2 \\
% & $\checkmark$ & $\checkmark$ & $\checkmark$ & 65.7 & 75.5 & 66.3 & \textbf{77.0} & 65.7 \\
\midrule

\multirow{3}{*}{DanceTrack} & $\checkmark$ & & &  \textbf{55.5} & \textbf{53.9} & \textbf{38.3} & 90.1 & \textbf{80.8} \\
& $\checkmark$ & $\checkmark$ & & 54.3 & 53.8 & 36.8 & 90.1 & 80.6  \\
& $\checkmark$ & & $\checkmark$ & 54.7 & 53.3 & 37.5 & 90.1 & 80.5 \\

\midrule

\multirow{3}{*}{SportsMOT} 
& $\checkmark$ & & &  \textbf{70.4} & 86.7 & \textbf{57.2} & \textbf{69.5} & 94.7 \\
& $\checkmark$ & $\checkmark$ & & 70.3 & \textbf{86.9} & 57.1 & 69.3 & \textbf{94.8} \\
& $\checkmark$ & & $\checkmark$ & 70.3 & 86.8 & 57.0 & 69.3 & 94.7 \\


\bottomrule
\end{tabular}
}
\vspace{-18pt}
\label{table:cost}
\end{center}

% \begin{center}
%     {
% \begin{tabular}{ccc|cccccc}
% % \toprule
% % \multicolumn{6}{c}{DanceTrack - Val} \\
% \toprule
%  \hspace{.5em}$IoU$\hspace{.5em} & \hspace{.5em}$L1$\hspace{.5em} & \hspace{.5em}$L2$\hspace{.5em} & HOTA & DetA & AssA & IDF1 & MOTA\\
% \midrule
% $\checkmark$ & & &  65.5 & 65.2 & 66.3 & 75.3 & 76.9 \\
% $\checkmark$ & $\checkmark$ & & \textbf{66.9} & \textbf{67.9} & \textbf{66.4} & \textbf{77.2} & 76.9 \\
% $\checkmark$ & & $\checkmark$ & 65.4 & 65.2 & 66.3 & 75.3 & 76.8 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}


\label{table:mot17-ablation}

\end{table*} 



==> table/mot17.tex <==
\begin{table}{r}{\linewidth}
\vspace{-26pt}
\caption{\textbf{Performance on MOT17.}}
  \begin{center}
    {\small{
\begin{tabular}{lccc}
\toprule

 Methods & HOTA & IDF1 & MOTA \\

\midrule
\textit{Kalman filter-based:} \\
SORT \cite{bewley2016simple} & 34.0 & 39.8 & 43.1 \\
FairMOT \cite{zhang2021fairmot} & 59.3 & 72.3 & 73.7 \\
ByteTrack \cite{zhang2022bytetrack} & 63.1 & 77.3 & 80.3 \\
OCSORT \cite{cao2023observation} & 63.2 & 77.5 & 78.0 \\
\midrule
\textit{Learning-based:} \\
CenterTrack \cite{zhou2020tracking} & 52.2 & 64.7 & 67.8\\
TraDes \cite{trades} & 52.7 & 63.9 & 69.1 \\
QDTrack \cite{fischer2023qdtrack}  & 53.9 & 66.3 & 68.7 \\
PermaTrack \cite{permatrack} & 55.5 & 68.9 & 73.8 \\
TransTrack \cite{sun2020transtrack} & 54.1 & 63.9 & 74.5 \\
TransCenter \cite{xu2021transcenter} & 54.5 & 62.2 & 73.2 \\
MeMOT \cite{cai2022memot} & 56.9 & 69.0 & 72.5 \\
MOTR \cite{zeng2022motr} & 57.2 & 68.4 & 71.9 \\
GTR \cite{zhou2022global} & 59.1 & 71.5 & 75.3 \\
MotionTrack \cite{xiao2023motiontrack} & 60.9 & 73.5 & 76.5 \\

\rowcolor{aliceblue}
MambaTrack & 60.5 & 72.3 & \textbf{78.2} \\

\rowcolor{aliceblue}
MambaTrack\textsuperscript{+} & \textbf{61.1} & \textbf{73.9} & 78.1 \\

\bottomrule
\end{tabular}
}}
\end{center}
\vspace{-16pt}
\label{table:mot17}
\end{table}

==> table/mot17_one_column.tex <==
\begin{table}[t]

\vspace{6pt}
\caption{\textbf{Performance on MOT17.} We compared our performance with different Kalman filter-based and learning-based methods using the official YOLO-X detections.}
  \begin{center}
\resizebox{0.55\linewidth}{!}{
\begin{tabular}{lccc}
\toprule

 Methods & HOTA & IDF1 & MOTA \\

\midrule
\textit{Kalman filter-based:} \\
SORT \cite{bewley2016simple} & 34.0 & 39.8 & 43.1 \\
FairMOT \cite{zhang2021fairmot} & 59.3 & 72.3 & 73.7 \\
ByteTrack \cite{zhang2022bytetrack} & 63.1 & 77.3 & 80.3 \\
OCSORT \cite{cao2023observation} & 63.2 & 77.5 & 78.0 \\
\midrule
\textit{Learning-based:} \\
CenterTrack \cite{zhou2020tracking} & 52.2 & 64.7 & 67.8\\
TraDes \cite{trades} & 52.7 & 63.9 & 69.1 \\
QDTrack \cite{fischer2023qdtrack}  & 53.9 & 66.3 & 68.7 \\
PermaTrack \cite{permatrack} & 55.5 & 68.9 & 73.8 \\
TransTrack \cite{sun2020transtrack} & 54.1 & 63.9 & 74.5 \\
TransCenter \cite{xu2021transcenter} & 54.5 & 62.2 & 73.2 \\
MeMOT \cite{cai2022memot} & 56.9 & 69.0 & 72.5 \\
MOTR \cite{zeng2022motr} & 57.2 & 68.4 & 71.9 \\
GTR \cite{zhou2022global} & 59.1 & 71.5 & 75.3 \\
MotionTrack \cite{xiao2023motiontrack} & 60.9 & 73.5 & 76.5 \\

\rowcolor{aliceblue}
MambaTrack & 60.5 & 72.3 & \textbf{78.2} \\

\rowcolor{aliceblue}
MambaTrack\textsuperscript{+} & \textbf{61.1} & \textbf{73.9} & 78.1 \\

\bottomrule
\end{tabular}
}
\end{center}
\vspace{-8pt}
\label{table:mot17-one-column}
\end{table}

==> tex/8_rebuttal.tex <==
We thank the reviewers for their valuable feedback and are pleased that MambaMOT was recognized for its ability to capture complex motions and outperform traditional Kalman filter-based methods. We also appreciate the acknowledgment of our clear writing and MambaMOT's innovative use of state-space models for motion prediction. We address the concerns raised in the reviews as follows.

\vspace{3pt}

\noindent\textbf{Inference Configuration.}
We conducted a fair comparison with the transformer-based tracker MOTR~\cite{zeng2022motr} under the same GPU hardware configuration. Our method achieves near real-time performance at 27.8 FPS, significantly outperforming MOTR, which achieves only 7.5 FPS. This demonstrates the efficiency of our method and its strong potential for real-world applications in tracking.

\vspace{3pt}

\noindent\textbf{SORT and DeepSORT Performance.}
We apologize for the confusion in our table and sincerely thank the reviewer for bringing this to our attention. We have modified the reference to the appropriate paper accordingly. The tracking performance of SORT~\cite{bewley2016simple} and DeepSORT~\cite{wojke2017simple} on DanceTrack~\cite{sun2022dancetrack} is faithfully reported from the experiments in prior work~\cite{cao2023observation}. DeepSORT integrates an additional deep appearance descriptor into the tracking process, which has proven effective in simpler datasets such as MOT17~\cite{milan2016mot16}, where each instance typically has distinct appearances. However, in the context of DanceTrack, where many targets have nearly identical appearances, relying heavily on appearance cues while reducing the emphasis on motion during the association stage can degrade performance further.

\vspace{3pt}

\noindent\textbf{Related Work on Mamba.} 
We thank the reviewer for the suggestion and will include a discussion of these Mamba-based methods in the final version of our paper. Unlike our MambaMOT, which focuses on the RGB modality for Multi-Object Tracking (MOT), MambaEVT~\cite{wang2024mambaevt} and Mamba-FETrack~\cite{mambafetrack} target event camera-based tasks, specifically Visual Object Tracking (VOT), which involves tracking a single object in a video. In contrast, our MambaMOT is tailored for tracking multiple objects simultaneously. Nonetheless, MambaMOT could potentially be adapted as a motion predictor to enhance the performance of VOT methods. A concurrent work, MambaTrack~\cite{xiao2024mambatrack}, employs a more complex design featuring bidirectional Mamba blocks and stacks additional layers with more parameters compared to our simpler design, which prioritizes simplifying the motion prediction for broader application scenarios. Additionally, MambaTrack solely focuses on motion modeling, while our proposed MambaMOT\textsuperscript{+} further extends functionality by leveraging motion features of each tracklet for global trajectory association.

\noindent\textbf{Inclusion of ID Switch.}
We appreciate the reviewer’s suggestion regarding the inclusion of ID switch in our evaluation, and we include the comparison of our proposed MambaMOT\textsuperscript{+} with other Kalman filter-based methods including ByteTrack~\cite{zhang2022bytetrack} and OC-SORT~\cite{cao2023observation} in Table~\ref{table:ids}. As shown in the table, MambaMOT\textsuperscript{+} outperforms popular Kalman filter-based methods including ByteTrack and OC-SORT in various metrics using the same detection generated by YOLOX~\cite{ge2021yolox}. 
% However, we note that ID switches are highly sensitive to occlusions and minor errors, often penalizing robust trackers unfairly. Metrics like AssA and IDF1 are considered more balanced for evaluating MOT performance.

\input{table/ids}
